CLDyB: Towards Dynamic Benchmarking for Continual Learning with Pre-trained Models

The advent of the foundation model era has sparked significant research interest in leveraging pre-trained representations for continual learning (CL), yielding a series of top-performing CL methods on standard evaluation benchmarks. Nonetheless, there are growing concerns regarding potential data contamination during the pre-training stage. Furthermore, standard evaluation benchmarks, which are typically static, fail to capture the complexities of real-world CL scenarios, resulting in saturated performance. To address these issues, we describe CL on dynamic benchmarks (CLDyB), a general computational framework based on Markov decision processes for evaluating CL methods reliably. CLDyB dynamically identifies inherently difficult and algorithm-dependent tasks for the given CL methods, and determines challenging task orders using Monte Carlo tree search. Leveraging CLDyB, we first conduct a joint evaluation of multiple state-of-the-art CL methods, leading to a set of commonly challenging and generalizable task sequences where existing CL methods tend to perform poorly. We then conduct separate evaluations of individual CL methods using CLDyB, discovering their respective strengths and weaknesses. The source code and generated task sequences are publicly accessible at https://github.com/szc12153/CLDyB.

==> sections/datasets.tex <==
\section{CLDyB Data Pool}
\label{sec:data_pool}
As we have discussed in Introduction and Fig.~\ref{fig: motivation}, image classification datasets, such as CIFAR-100~\citep{krizhevsky2009learning}, CUB-200~\citep{wah2011caltech} and Stanford Cars~\citep{krause20133d} have been commonly used for the evaluation of CL strategies, but they have their respective limitations. 
% For example, 
% the data of these datasets are 1) \textcolor{red}{some limitations}. 
To solve these limitations, we propose an initial strategy that dynamically assesses CL models by searching a series of tasks from a large data pool. In this section, we will introduce the building of the data pool, CLDyB-pool. It includes a diverse collection of real-world datasets for the primary experiments, as well as several generated datasets for additional explorations. There are a total of 26 datasets, including 2,505,185 images across 2,403 categories. The details are as follows.
% 2,461,342 real-world $+$ 43843 generated images from 2043 (real-world)  $+$ 500 categories. CLDyB-pool contains two types of data.


% Total Images: 2461342
% Total Classes: 2043
% Total Datasets: 22

% Class Stats:

% Dataset Stats:
% Dataset: Sea, Count: 13711
% Dataset: aircraft, Count: 10000
% Dataset: EuroSAT_RGB, Count: 27000
% Dataset: Indian_Food, Count: 4000
% Dataset: Oxford5k, Count: 5063
% Dataset: Apparel, Count: 16170
% Dataset: Butterfly, Count: 6499
% Dataset: CNFOOD241, Count: 170835
% Dataset: foodX251, Count: 118441
% Dataset: Rock, Count: 3687
% Dataset: Sports100, Count: 13492
% Dataset: Fruits_Vegetable, Count: 3047
% Dataset: SUN397, Count: 17355
% Dataset: Jute_Pest, Count: 7151
% Dataset: Animal, Count: 5400
% Dataset: RESISC45, Count: 5100
% Dataset: food101, Count: 101000
% Dataset: One_piece, Count: 11737
% Dataset: MLRSNet, Count: 109161
% Dataset: Balls30, Count: 3708
% Dataset: Clothing, Count: 5325
% Dataset: Places365, Count: 1803460

% Unique Class Count Per Dataset:
% Dataset: Sea, Unique Classes: 23
% Dataset: aircraft, Unique Classes: 100
% Dataset: EuroSAT_RGB, Unique Classes: 10
% Dataset: Indian_Food, Unique Classes: 80
% Dataset: Oxford5k, Unique Classes: 17
% Dataset: Apparel, Unique Classes: 37
% Dataset: Butterfly, Unique Classes: 75
% Dataset: CNFOOD241, Unique Classes: 240
% Dataset: foodX251, Unique Classes: 250
% Dataset: Rock, Unique Classes: 9
% Dataset: Sports100, Unique Classes: 100
% Dataset: Fruits_Vegetable, Unique Classes: 35
% Dataset: SUN397, Unique Classes: 339
% Dataset: Jute_Pest, Unique Classes: 17
% Dataset: Animal, Unique Classes: 90
% Dataset: RESISC45, Unique Classes: 45
% Dataset: food101, Unique Classes: 101
% Dataset: One_piece, Unique Classes: 18
% Dataset: MLRSNet, Unique Classes: 46
% Dataset: Balls30, Unique Classes: 29
% Dataset: Clothing, Unique Classes: 17
% Dataset: Places365, Unique Classes: 365


% Total Images: 43843
% Total Classes: 360
% Total Datasets: 4

% Class Stats:

% Dataset Stats:
% Dataset: Product100, Count: 7095
% Dataset: Animal2, Count: 19962
% Dataset: Animal_sketch, Count: 8494
% Dataset: Animal, Count: 8292

% Unique Class Count Per Dataset:
% Dataset: Product100, Unique Classes: 71
% Dataset: Animal2, Unique Classes: 133
% Dataset: Animal_sketch, Unique Classes: 77
% Dataset: Animal, Unique Classes: 79



\textbf{Real-world data.} The CLDyB-pool real-world data inludes 2,043 classes from 22 publicly available image classification datasets. Subjects of these datasets have a broad distribution, including animals, plants, scenes, food, etc. The subjects across two major aspects within the CLDyB-pool: 1) Natural and Biological Sciences include classes of fauna, flora and other natural elements and ecosystems. These subjects cover various levels of granularity, from coarse-grained, such as different categories of animals from Animal-90~\citep{banerjee_animal_image_2024}, to fine-grained categories, such as various classes of butterflies from Butterfly-70~\citep{phucthai_butterfly_image_2024},  2) Human-Made Objects/Scenes contain images of clothing, food, buildings, and entertainment scenes. This group also captures multi-national and multicultural diversity, highlighting historical diversity across different regions and eras. For example, we have food classes from Food-101~\citep{bossard2014food}, CNFOOD-241\citep{zachaluza_cnfood_2024} (Chinese cuisine), Indian Food Images \citep{banerjee_indian_food_2023} etc., datasets. which includes cuisines of a variety of regions and cultures.
% Based on these datasets, the search task series can include data from different 
%
% \textcolor{red}{It is important to highlight that datasets commonly used for CL tasks are typically from a single set, like CUB~\cite{}.} In comparison,
By involving data from the two aspects, CLDyB-pool includes a wider range of domains and diverse classes, offering broader distribution coverage, thus offering an ideal test platform for CL methods. 



% \begin{figure}[t]
%   \centering
%   \fbox{\rule[-.5cm]{0cm}{3cm} \rule[-.5cm]{4cm}{0cm}}
%   % \includegraphics[width=1.\linewidth]{fig/datapool.pdf}
%   \caption{ 
% \textbf{Subjects, statistics and examples of CLDyB-pool. We divided all classes in the data pool into two groups (A) Natural and Biological Sciences and (B)Human-Made Objects/Scene }. 
% }
% \vspace{-1em}
% \label{fig:fig-data-pool}
% \end{figure}

\textbf{Diffusion mode generated data.} CLDyB-pool includes 4 datasets generated by SDXL~\citep{podellsdxl}. Specifically, 360 classes of three animal and one product datasets are generated by using prompts `\textit{A high-quality image of a kind of animal: $\{$animal name$\}$}', `\textit{A high-quality sketch image of a kind of animal: $\{$animal name$\}$}', `\textit{A high-quality $\{$image style$\}$ image of a kind of animal: $\{$animal name$\}$}' and `\textit{A high-quality image of a kind of product: $\{$product name$\}$}'. Incorporating the generated data will expand the CLDyB pool to include additional distributions, leading to more challenging task series (we will discuss in Section~\ref{sec: additional-ana}).

Additional details about the CLDyB-pool can be found in the Appendix~\ref{sec: app-datasets}. We will use the CLDyB-pool as a dynamic source to dynamically search for task series. We expect that CLDyB-pool will be valuable for ongoing research in continual learning and beyond. In the future, our goal is to develop CLDyB-pool into a dynamic online project through open-source collaboration with the community.


[Consider moving this paragraph under Section 4] \textbf{Time-evolving data pool}~$\quad$~\chen{need to metnion some ideas on how should we udpate the dataset in the pool based on the current results of task-selection? For example, picking visually/conceptually similar datasets to those often selected by our dynamic task selection pipeline ?}

==> sections/iclr_instructions.tex <==

\section{Submission of conference papers to ICLR 2024}

ICLR requires electronic submissions, processed by
\url{https://openreview.net/}. See ICLR's website for more instructions.

If your paper is ultimately accepted, the statement {\tt
  {\textbackslash}iclrfinalcopy} should be inserted to adjust the
format to the camera ready requirements.

The format for the submissions is a variant of the NeurIPS format.
Please read carefully the instructions below, and follow them
faithfully.

\subsection{Style}

Papers to be submitted to ICLR 2024 must be prepared according to the
instructions presented here.

%% Please note that we have introduced automatic line number generation
%% into the style file for \LaTeXe. This is to help reviewers
%% refer to specific lines of the paper when they make their comments. Please do
%% NOT refer to these line numbers in your paper as they will be removed from the
%% style file for the final version of accepted papers.

Authors are required to use the ICLR \LaTeX{} style files obtainable at the
ICLR website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsection{Retrieval of style files}

The style files for ICLR and other conference information are available online at:
\begin{center}
   \url{http://www.iclr.cc/}
\end{center}
The file \verb+iclr2024_conference.pdf+ contains these
instructions and illustrates the
various formatting requirements your ICLR paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+iclr2024_conference.sty+ and \verb+iclr2024_conference.bst+ (to be used with \LaTeX{}2e). The file
\verb+iclr2024_conference.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).
Use 10~point type with a vertical spacing of 11~points. Times New Roman is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, in small caps and left-aligned.
All pages should start at 1~inch (6~picas) from the top of the page.

Authors' names are
set in boldface, and each name is placed above its corresponding
address. The lead author's name is to be listed first, and
the co-authors' names are set to follow. Authors sharing the
same address can be on the same line.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.


There will be a strict upper limit of 9 pages for the main text of the initial submission, with unlimited additional pages for citations. 

\section{Headings: first level}
\label{headings}

First level headings are in small caps,
flush left and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are in small caps,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in small caps,
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textsc{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.

\subsubsection*{Author Contributions}
If you'd like to, you may include  a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors.

\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.

==> sections/method_old_to_keep.tex <==
\section{Dynamic Benchmarking for Continual Learning}

\label{sec:pipeline}

Our objective is primarily to facilitate rapid algorithm development within the continual learning community while also providing a framework that enhances the likelihood of algorithmic developments made with our benchmark translating into strong real-world performance.
In this section, we describe the two stages of our benchmarking framework, referred to as the \textbf{CLDyB-pipeline}, as shown in Fig.~\ref{fig: pipeline}, i.e., sampling difficult tasks and searching for difficult task sequences, each corresponding to the two key challenges outlined in the Introduction.

\begin{figure}[b!]
\centering
\includegraphics[width=\linewidth]{fig/pipeline7.pdf}
\caption{An overview of the proposed two-stage \textbf{CLDyB-pipeline} for dynamically constructing challenging task sequences to the $M$ CL models $\mathcal{F}^{(t-1)}$, at each time step $t$. \textbf{Stage A}: Initially, the CLDyB-pipeline generates $|\mathcal{T}^{(t)}_{(g)}|$ intrinsically difficult tasks (Eqn.~(\ref{eq:ats})) from a potentially time-evolving data pool. These candidates are then clustered based on the functional skills required for accurate classification, ensuring a comprehensive range of diverse tasks in the serach space $\mathcal{T}^{(t)}$. \textbf{Stage B}: Monte Carlo tree search is employed to estimate the values (Eqn.~(\ref{eq:search_objective})) of the tasks in $|\mathcal{T}^{(t)}|$. The task with the highest value is selected as the $t$-th task for all CL models to learn and evaluate, resulting in the updated task sequence $\mathcal{T}^{<(t+1)}=\mathcal{T}^{<(t)}\cup\mathcal{T}^{(t)}$ and CL models $\mathcal{F}^{(t)} = \{\mathtt{A}_m(f_m^{(t-1)},\mathcal{T}^{(t)})\}^{M}_{m=1}$. Pseudocodes can be found in Alg.~\ref{alg:pscode-cldy-pipeline}.}
\label{fig: pipeline}
\end{figure}

\subsection{Towards Intra-task Difficulty -- Sampling Difficult Tasks}\label{sec: greed_task_sampling}
When the tasks used for continual learning of a pre-trained model \chen{largely} overlap with the pre-training data, the resulting high performance is unsurprising and fails to fairly evaluate the effectiveness of CL algorithms~\citep{pmlr-v232-galashov23a}, \chen{as data contamination is the \textit{dominant contributor} to high performance}.
To avoid such data contamination while simultaneously challenging the continually learned model, our first goal is to \emph{construct continual learning tasks that are intrinsically and individually difficult to the evolving CL model $f^{(t)}_m$ at each step $t$, including for the pre-trained model $f^{(0)}_m$}.
Provided with a pool of classes, one straightforward recipe to screening difficult classification tasks involves: (1) randomly sampling $K$ classes with equal probability from the pool to form a task, (2) repeating step (1) to enumerate as many tasks as possible, and (3) selecting tasks that exceed a predefined difficulty threshold.
Unfortunately, due to the vast size of the data pool which we will detail in Appendix~\ref{sec:data_pool} and the frequency of task screening (performed at every step $t$), this approach turns prohibitively~expensive. 


\textbf{Greedy task sampling} $\quad$ To significantly reduce the complexity, we turn to directly sample $|\mathbb{T}^{(t)}_{(g)}|$ most probably difficult tasks $\mathbb{T}^{(t)}_{(g)}$, where the sampling probability of a task $p^{(t)}(\mathcal{T})$ is naturally a joint distribution over $K$ classes. 
By formulating this joint distribution with Markov Random Field~\citep{Sherrington1975SolvableMO} and leveraging the observation that the difficulty of a multi-class classification task closely relates to the separability between pairs of classes ~\citep{He_2020_CVPR}, we define the sampling probability as proportional to the product of class pairwise potential functions, i.e., 
\begin{equation}\small
      p^{(t)}(\mathcal{T})\propto \prod_{p,q\in\{1,\cdots,K\}} \Psi(\mathcal{C}_p,\mathcal{C}_q ),\quad \Psi(\mathcal{C}_p,\mathcal{C}_q ) = \frac{1}{M}\sum_{m=1}^{M}\boldsymbol{z}(\text{cos}(\boldsymbol{\mu}^{(t-1)}_{m,p},\boldsymbol{\mu}^{(t-1)}_{m,q})).\label{eq:ats}
\end{equation}
The operator $\boldsymbol{z}(\cdot)$ denotes the min-max normalization  $\frac{(\cdot)-\min(\cdot)}{\max(\cdot)-\min(\cdot)}\mapsto [0, 1]$, and $\text{cos}(\cdot,\cdot)$ represents cosine similarity. Here, $\boldsymbol{\mu}^{(t)}_{m,p}$ represents the prototype for class $p$ according to the features extracted via $f^{(t-1)}_{m}$.
This sampling probability thus targets the identification of the most difficult tasks that challenge the current feature space's capacity -- a task involving more challenging pairwise class discrimination, reflected in the higher value of the pairwise potential product, is assigned greater sampling probability for its corresponding $K$ classes. \chen{See Appendix~\ref{app: heuristic} for more discussion.}

Inspired by pairwise random field based image segmentation~\citep{kohli2013principled}, we propose to sample $K$ classes that maximize $p^{(t)}(\mathcal{T})$ through a greedy algorithm, where classes from each task are selected sequentially.
Initially, the first class is uniformly sampled from the entire set of available classes in our data pool $\mathcal{D}$, ensuring that the selected tasks in $\mathbb{T}^{(t)}_{(g)}$ exhibit sufficient diversity.
Subsequently, during each $k$-th iteration of the greedy process, we choose the class $\hat{p}$ that contributes the maximum increase in the product of potentials, i.e., $\hat{p} = \arg\max_p\prod_{q\in\{1,\cdots,k-1\}}\Psi(\mathcal{C}_p,\mathcal{C}_q)$. 
The greedy sampling continues until $K$ distinct classes are sampled.
We repeat this greedy process $|\mathbb{T}^{(t)}_{(g)}|$ times. 
%for each $m$-th CL model and iterate over all $M$ models, completing the whole set $\mathbb{T}^{(t)}=\cup_{m=1}^M \mathbb{T}^{(t)}_{m}$ of sampled tasks.
Detailed procedures are available in Alg.~\ref{alg:pscode_ts}.


% To tackle this issue, we utilize an adaptive task sampling approach to build the task space $\mathcal{T}^{(t)}$ from a pool of available classes at each time step, dynamically. Here, each task within $\mathcal{T}^{(t)}$ is characterized as an N-way classification problem with disjoint training, validation, and testing set samples, independently drawn from the combined N class-conditional data-generating distributions. For each class, we first determine the pair-wise class potential $C^{(t)}(i,j)$ by leveraging the continual learning models trained up to the current point in time, forming a complete and undirected graph. We specify $C^{(t)}(i,j)$ as
% \begin{equation}
%    C^{(t)}(i,j):=-\frac{1}{M}\sum_{m=1}^{M}\mathbb{E}_{i'\sim i,j'\sim j}[\tilde{l}_2^m(f^m(x_{i'}),f^m(x_{j'}))],
% \end{equation}
% where $\tilde{l}_2^m$ represents the normalized $l_2$ distance within the range $[0,1]$ for the $m$-th learner defined by $\frac{(\cdot)-\min l_2^m}{\max l_2^m-\min l_2^m}$, and consequently, $C^{(t)}(i,j)$ serves as a similarity metric between class $i$ and class $j$ at time $t$. We then sample N classes as a task with a probability proportional to their N-cliques potentials, which is expressed as
% \begin{equation}
%     P(\mathcal{T})\propto \prod_{i,j\in\mathcal{T}}C^{(t)}(i,j).
% \end{equation}
% We sample $K$ such tasks to build $\mathcal{T}^{(t)}$ at each time step $t$.

\textbf{Functional task clustering}$\quad$
The set of sampled tasks $\mathbb{T}^{(t)}_{(g)}$ from the previous step is likely to exhibit (1) a biased distribution of tasks across the functional skills necessary for accurate classification, and (2) redundancy.
%A na\"ive merging of the $M$ sampled task sets $\mathbb{T}^{(t)}_1,\cdots,\mathbb{T}^{(t)}_M$ likely leads to a biased distribution of tasks over functional skills required for successful classification. 
This occurs because the $M$ CL models naturally fall into different clusters based on their functional skills. 
Consequently, uniform task sampling tends to favor those tasks associated with the models belonging to the dominant functional skill cluster, which contradicts our goal of covering task candidates that challenge $M$ CL models equally. 
To address this issue, we propose further clustering tasks based on their functional skills required and adopting an ancestral sampling approach to fill a reduced candidate set $\mathcal{T}^{(t)}$ with $|\mathcal{T}^{(t)}|\leq|\mathcal{T}^{(t)}_{(g)}|$. We first uniformly sample a cluster and then draw a task from the chosen cluster.
To create these clusters, we construct an $M$-dim functional vector for each task by evaluating the negative log-likelihood~(NLL) of each sampled task under $M$ $k$-NN classifiers derived from the CL models $\mathcal{F}^{(t-1)}_m$.
The clusters are then formed using a standard $k$-means algorithm. Pseudocodes are provided in Alg.~\ref{alg:pscode_ftc}.

\subsection{Towards Inter-task Difficulty -- Searching for Difficult Task Sequences}
The primary challenge in continual learning arises from its non-stationary nature, where tasks encountered in the wild are non-\emph{i.i.d.} and previously unseen~\citep{verwimp2024continuallearningapplicationsroad}.
As a result, even algorithms that perform quite well on current static benchmarks remain susceptible to real-world tasks, accompanied with either severe forgetting or negative transfer.
For less overfitting to static benchmarks, our second goal is to \emph{dynamically construct continual learning task sequences that pose significant challenges to $M$ CL models across all time steps, i.e., by maximizing forgetting and minimizing plasticity}. Mathematically, 
% \subsection{Problem Formulation}
% Our objective in benchmark design is to address the \chen{three aforementioned challenges in the introduction}. First, to prevent data contamination when using strong pre-trained models, we argue that the CL task sequences should be sufficiently challenging. 
%To prevent data contamination when using powerful pre-trained models for CL, the reward function for task selection is intentionally designed to in opposition to the general objectives of CL algorithms, which are to minimize forgetting and maximize forward transfer. Thus, our proposed pipeline always challenges the CL algorithms by aiming to obtain their worst-case performance over a CL task sequence, making the results of our evaluation indicative of the robustness of the CL algorithms. 
% Specifically, 
for a sequence of $N$ tasks, we formulate and solve the following optimization problem to identify these challenging sequences in a model-based manner, % in a model-based manner, %, mathematically expressed as
\begin{equation}\small
\mathcal{T}^{<(N+1)}= %\argmax_{\tilde{\mathcal{T}}^{<(N+1)}\in\boldsymbol{\pi}}R(\mathcal{F}^{(N)},\tilde{\mathcal{T}}^{N+1})=
\argmax_{\tilde{\mathcal{T}}^{<(N+1)}\in\boldsymbol{\pi}}\mathtt{AFM}(\tilde{\mathcal{T}}^{<(N+1)},\mathcal{F}^{(N)}) - \mathtt{ALA}(\tilde{\mathcal{T}}^{<(N+1)},\mathcal{F}^{(N)}) \label{eq:ori_objective},
\end{equation}
where $\boldsymbol{\pi}$ is the set of all possible ordered task sequences. Note that our goal for task sequence construction in Eqn.~(\ref{eq:ori_objective}) opposes the general objectives of CL algorithms, which are to minimize forgetting and maximize learning plasticity.
Intuitively, the stronger the CL algorithms (and models), the fewer weaknesses they will have, and the higher their performance will be when subjected to the adversarial task sequence constructed from Eqn.~(\ref{eq:ori_objective}). Thus, the results of our evaluation  provide insights into the robustness of CL algorithms. This helps reveal the shortcomings of state-of-the-art CL algorithms, and yield valuable training and assessment data which the CL community can leverage to develop even stronger algorithms.
\par
%  Mathematically, let $\mathcal{T}$ represent the entire task space, and let $\pi(\gS,l)$ be the set of all permutations of length $l$ of elements in a set $\gS$ (all uniquely ordered arrangements of $l$ elements in $\gS$). Our goal is to determine the optimal task sequence (i.e., a particular permutation) $T:=\mathcal{T}_1,\mathcal{T}_2,\ldots,\mathcal{T}_L$ that minimizes the performance of $M$ given continual learning algorithms, expressed as:
% \begin{equation}
% T^*:=\argmin_{T'\in\pi(\mathcal{T},l)}\sum_{m=1}^{M}\gV(\mathtt{A}_m,T') \label{eq:ori_objective}
% \end{equation}
% where $\gV(\mathtt{A}_m,T')$ quantifies the performance of a continual learning algorithm $\mathtt{A}_m$ on the task sequence $T'$.

% At high level, to reduce overfitting to static benchmarks, our evaluation protocol should dynamically choose the next CL task at each time $t$ based on the current states of the trained models to maximize some reward. The CL models are then trained on the chosen task and evaluated on the entire sequence of tasks, mirroring the setups in standard CL, with this procedure repeating indefinitely.

% In a conventional CiCL benchmark, task sequences are generated by randomly dividing a labelled dataset $\sD$ into multiple subsets with disjoint class labels, followed by randomly permuting the order of these subsets. Thus, $\boldsymbol{\pi}$ is the product space of permutations and combinations, which is enormous and discrete. Additionally, evaluating $\mathtt{Fgt}$ and $\mathtt{Fwt}$ in the objective necessitates unrolling a total of $N$ time steps in CL, which involves iteratively training the $M$ models on the $N$ tasks. As a result, solving for an off-line global optimal in Eqn.~(\ref{eq:ori_objective}) becomes practically infeasible.\par

Eqn.~(\ref{eq:ori_objective}), however, is an offline optimization problem, and the global maximal depends on the sequence length $N$ - which is an unknown variable or potentially infinite in real-world CL applications. To this end, we reformulate Eqn.~(\ref{eq:ori_objective}) into an online sequential decision-making problem as shown in Eqn.~(\ref{eq:dp_objective}). Concretely, we consider the CL algorithms as a deterministic stationary discrete-time
system of the form $\mathcal{F}^{(t)} = \{\mathtt{A}_m(f_m^{(t-1)},\mathcal{T}^{(t)})\}^{M}_{m=1}$, which defines a state transition function from observable state $\mathcal{F}^{(t-1)}$ to $\mathcal{F}^{(t)}$ under action 
%is the observable state and the task $\mathcal{T}^{(t)}\in 
$\mathcal{T}^{(t)}$ returned by our task selection policy $\mathtt{A}^\mathtt{CLDyB}$ , i.e., $\mathcal{T}^{(t)} = \mathtt{A}^\mathtt{CLDyB}(\mathcal{F}^{(t-1)})$, at time $t$. Defining the \textbf{immediate reward} function after transition from $\mathcal{F}^{(t-1)}$ to $\mathcal{F}^{(t)}$ with action $\mathcal{T}^{(t)}$ as $R(\mathcal{F}^{(t-1)},\mathcal{T}^{(t)})=\mathtt{AFM}(\tilde{\mathcal{T}}^{<(t+1)},\mathcal{F}^{(t)}) - \mathtt{ALA}(\tilde{\mathcal{T}}^{<(t+1)},\mathcal{F}^{(t)})$, and the value function of $\mathtt{A}^{\mathtt{CLDyB}}$ at the initial state as $Q_{\mathtt{A}^{\mathtt{CLDyB}}}(\mathcal{F}^{(0)})$, 
% as $Q(\mathcal{F}^{(0)})$,
we aim to find an optimal policy $\mathtt{A}^\mathtt{CLDyB}$, hence sequences of optimal actions under $\mathtt{A}^\mathtt{CLDyB}$, that maximizes this value function, that is
\begin{equation}\small
    \mathcal{T}^{<(N+1)} = \{\mathcal{T}^{(t)}=\mathtt{A}^{\mathtt{CLDyB}}(\mathcal{F}^{(t-1)})\}^{N}_{t=1};~\textrm{s.t.}~ \mathtt{A}^{\mathtt{CLDyB}}=\argmax_{\tilde{\mathtt{A}}^{\mathtt{CLDyB}}}\underbrace{\lim_{N\to\infty} \sum_{t=1}^{N}\alpha^{t-1}R(\mathcal{F}^{(t-1)},\tilde{\mathtt{A}}^{\mathtt{CLDyB}}(\mathcal{F}^{(t-1)}))}_{Q_{\tilde{\mathtt{A}}^{\mathtt{CLDyB}}}(\mathcal{F}^{(0)})}, \label{eq:dp_objective}
\end{equation}


where $\alpha\in(0, 1]$ is a discount factor. 
Solving the above optimization problem presents two key challenges, including (1) accurately estimating the value function, which can vary significantly by CL algorithms and task properties (e.g., the number of classes in a task) and (2) efficiently navigating the vast and discrete search space, which is compounded by the large number of tasks $|\mathcal{T}^{(t)}|$ at each time step and the considerable length of the task sequence.


% In the following sections, we propose a simple dynamic task selection pipeline that incorporates a series of approximations to solve for $\mathcal{T}^{N+1}$ effectively and tractably. 
%The high-level idea of our pipeline is illustrated in Fig.~\ref{fig: pipeline} and the pseudocode of the algorithm is provided in \Secref{app:pcode_ts}.


% Solving the optimization problem in Eqn.~(\ref{eq:ori_objective}) can be pr
% provides a straightforward formulation of our problem of interest, addressing Eqn.~(\ref{eq:ori_objective}) to find a global optimum in a continual learning context can be notably difficult for the following two major reasons: 1) assessing the performance measure $\gV(\mathtt{A}_m,T')$ (such as final average accuracy or forgetting) generally necessitates repeatedly executing the algorithm $\mathtt{A}_m$ over the tasks in $T'$ for training purposes, and 2), the solution space $\pi(\gS,l)$ is vast and expands exponentially with increase of both the task sequence length $l$ and the task space $\mathcal{T}$. These potentially make solving the optimization problem  prohibitively computational expensive. \chen{In addition to the high computation demand, Eqn.(~\ref{eq:ori_objective}) is static/offline/too restrictive, it is not suitable for a dynamic evaluation settings where the length $l$ can potentially grows (to infinity) as a new task can be added at any time in future.}\par

 % To simplify the problem (\chen{or more accurately, to integrate dynamics into our benchmark design}), we reformulate the challenge of identifying a difficult task sequence as a two-player, online, sequential game. In this game, we act as the task selector (player one), while our adversaries are a collection of continual learning algorithms (player two). At each time step in the game, the task selector dynamically chooses the next task from $\mathcal{T}$ for the learners to train on and be assessed based on their current observable states. Once a task is chosen, all $M$ algorithms are applied on the selected task, with the objectives of minimizing forgetting of previous tasks and accelerate learning for future tasks - mirroring the standard continual learning training setup. This process generates observable model states for the next round of task selection. These two steps are repeated continually or until the selected task sequence $T$ reaches a specified length $L$. Our objective is to craft the dynamic task selector.\par

% \begin{algorithm}[h!]
%    \caption{SMAT: \textbf{Meta-testing time full fine-tuning} using $\theta_i$ as an model initialization (for a single task $\tilde\mathcal{T}_i$)}
%    \label{alg:collapse_then_full}
% \begin{algorithmic}
% \mathcal{T}ATE {\bfseries Input:} Testing support set $\tilde\mathcal{T}_i^s$ and query inputs $\tilde{\mathbf{X}}_i^q$; Meta-trained $\zeta,\theta^\delta,\Phi$, Pre-trained $\theta^\mathtt{pre}$ 
%     \mathcal{T}ATE $\boldsymbol{\alpha}_i'\sim \mathtt{GumbleSigmoid}(h_\zeta(\tilde\mathcal{T}^s_i))$ \Comment{Obtain expert merging scores using the hypernetwork}
%     \mathcal{T}ATE $\alpha_{i,m} = \frac{\alpha_{i,m}'}{\sum_m^{M}\alpha_{i,m}'}$ \Comment{Normalize the merging weights}
%         \mathcal{T}ATE $\boldsymbol{\theta}_i = \boldsymbol{\theta}^\mathtt{pre} +  \boldsymbol{\theta}^{\delta}\odot\sum_{m}^{M}\alpha_{i,m}\boldsymbol{z}_m$ \Comment{Weighted-sum of sparse experts}
%         \mathcal{T}ATE $\boldsymbol{\theta}_{i,0} \leftarrow\mathtt{StopGrads}(\boldsymbol{\theta}_i)$
%         \FOR{$k=0,2,...(K-1)$} 
%             \mathcal{T}ATE $\boldsymbol{\theta}_{i,k+1}\leftarrow\mathtt{GradientDescent}(\nabla_{\boldsymbol{\theta}_{i,k}}\gL_{\tilde\mathcal{T}_i^s}^\mathtt{ce}\boldsymbol{\theta}_{i,k})$ \Comment{finetune $\theta_{i}$ on the support set for $K$ steps}
%         \ENDFOR
% \mathcal{T}ATE  {\bfseries Return:} Final prediction on the query set $\hat{\mathbf{Y}}^{q}_i=f(\tilde{\mathbf{X}}_i^q;\boldsymbol{\theta}_{i,K})$
% \end{algorithmic}
% \end{algorithm}


% \subsection{Dynamic Task Selection}

\textbf{Tree search with approximation in value}$\quad$
Monte Carlo tree search (MCTS)~\citep{coulom2006efficient} is one of the widely-adopted solutions for online sequential decision-making problems~\citep{Puterman1994MarkovDP}, particularly well-suited to our CL setup due to its desirable ability in calculating value functions focused on a particular initial state on the fly. 
% Dynamic programming problems have been extensively studied and various solutions are available~\chen{cite}. In this work, we use a straightforward tree search algorithm, such as Monte Carlo tree search (MCTS)~\chen{cite}, to plan out optimal actions at each step in an online manner during CL. 
MCTS utilizes Monte Carlo simulations to approximate the value $Q_{\mathtt{A}^{\mathtt{CLDyB}}}(\mathcal{F}^{(t)})$ of each state $\mathcal{F}^{(t)}$ in a search tree. 
In each action round, MCTS alternates between four steps: (1) rollout simulation, where it performs simulations that expand the tree recursively to estimate the current state value until a predefined simulation budget is exhausted; (2) update, where the action values and visit counts of all preceding states associated with the current state are updated; (3) selection, where the action (i.e., task $\mathcal{T}^{(t)}$) leading to the state with the highest immediate value is chosen; and (4) expansion, where all CL algorithms learn on the selected task (the chosen action) and transit from the current state $\mathcal{F}^{(t-1)}$ to the next state $\mathcal{F}^{(t)}$.
% and updates corresponding state value estimates until a simulation budget of $K$ is exhausted. The optimal action for the current round is chosen by selecting the action leading to the state with the highest immediate value according to the tree.\par

Unfortunately, in a CL setup, MCTS simulations are resource-intensive due to (a) the necessity for performing an $(N-t)$-step rollout to evaluate the value function $Q_{\mathtt{A}^{\mathtt{CLDyB}}}(\mathcal{F}^{(t)})$, which involves training models on tasks at all $(N-t)$ steps, and (b) the indeterminate and potentially infinite termination length $N$ in an open-ended CL experiment. To mitigate these issues, we substitute the exact value function with the sum of the immediate reward and an $l$-step look-ahead reward. The hyperparameter $l$ mediates the trade-off between approximation bias and computational cost, allowing us to solve for a suboptimal action at each $t$ as
 \vspace{-2mm}
\begin{equation}
% \vspace{-5mm}
\small
      \mathcal{T}^{(t)}=\argmax_{\tilde{\mathcal{T}}^{(t)}\in\mathcal{T}^{(t)}}Q_{\tilde{\mathcal{T}}^{(t)}}(\mathcal{F}^{(t-1)})\approx \argmax_{\tilde{\mathcal{T}}^{(t)}\in\mathcal{T}^{(t)}}R(\mathcal{F}^{(t-1)},\tilde{\mathcal{T}}^{(t)}) + \sum_{l'=0}^{l-1}R(\mathtt{A}(\mathcal{F}^{(t-1+l')},\tilde{\mathcal{T}}^{(t+l')}),\tilde{\mathcal{T}}^{(t+l'+1)}).\label{eq:search_objective}
\end{equation}
For simplicity, we set $l=1$ and defer the use of more advanced techniques for value function approximation, such as learning a value network~\citep{Silver2016MasteringTG}, for future work. 
% In a typical CiCL benchmark, tasks are created by randomly partitioning a labelled dataset $\sD$ into several subsets with disjoint class labels~\chen{cite}. Consequently, the permissible action space $\boldsymbol{\pi}$ at each stage, encompassing combinations of all unseen classes within $\sD$, is vast and discrete, rendering exhaustive search impractical. To mitigate this issue, our subsequent objective is to constrain the action search space. \par

% \textbf{Adaptive task sampling}$\quad$Recognizing that not all tasks are equally challenging~(in terms of Eqn.~(\ref{eq:ori_objective})) for CL algorithms, e.g.,~\chen{cite}, we propose orienting the search towards more intrinsically difficult tasks at each step $t$. For classification, we postulate that the intrinsic difficulty of a CL task is proportional to the product of its pairwise class similarity as evaluated by $\mathcal{F}^{(t)}$. When expanding the tree, we restrict the original search space to a set $\mathcal{T}^{(t)}$ of $J$ difficult tasks, $J\ll|\boldsymbol{\pi}|$, through sampling, that is $ \mathcal{T}^{(t)}=\{\mathcal{T}_j\}_{j=0}^{J-1}\mathcal{T}ackrel{P^{(t)}(\mathcal{T})}{\sim}\boldsymbol{\pi}$, where
% \begin{equation}
%       P^{(t)}(\mathcal{T})\propto \prod_{p,q\in\mathcal{T}}C^{(t)}(p,q),\quad C^{(t)}(p,q)=\frac{1}{M}\sum_{m=1}^{M}\boldsymbol{z}(\cos(\mu^{(t)}_{m,p},\mu^{(t)}_{m,q})).\label{eq:ats}
% \end{equation}
% The operator $\boldsymbol{z}(\cdot)$ denotes the min-max normalization mapping to the interval $[0, 1]$ through $\frac{(\cdot)-\min(\cdot)}{\max(\cdot)-\min(\cdot)}$, $\mu^{(t)}_{m,p}$ represents the prototype for class-$p$, derived from the features obtained via $f^{(t)}_{m}$. Conceptually, a task that is initially more difficult will require more substantial updates to the CL models to achieve satisfactory performance, which may consequently result in increased forgetting. This task sampling strategy is realized through a greedy algorithm in which classes of a task are sampled sequentially one after another~(see Alg.~(\ref{alg:X}) for more details). To promote diversity in the feature representation of sampled tasks, the first class of each task is uniformly chosen from all the classes available in $\sD$.  \par

% % To tackle this issue, we utilize an adaptive task sampling approach to build the task space $\mathcal{T}^{(t)}$ from a pool of available classes at each time step, dynamically. Here, each task within $\mathcal{T}^{(t)}$ is characterized as an N-way classification problem with disjoint training, validation, and testing set samples, independently drawn from the combined N class-conditional data-generating distributions. For each class, we first determine the pair-wise class potential $C^{(t)}(i,j)$ by leveraging the continual learning models trained up to the current point in time, forming a complete and undirected graph. We specify $C^{(t)}(i,j)$ as
% % \begin{equation}
% %    C^{(t)}(i,j):=-\frac{1}{M}\sum_{m=1}^{M}\mathbb{E}_{i'\sim i,j'\sim j}[\tilde{l}_2^m(f^m(x_{i'}),f^m(x_{j'}))],
% % \end{equation}
% % where $\tilde{l}_2^m$ represents the normalized $l_2$ distance within the range $[0,1]$ for the $m$-th learner defined by $\frac{(\cdot)-\min l_2^m}{\max l_2^m-\min l_2^m}$, and consequently, $C^{(t)}(i,j)$ serves as a similarity metric between class $i$ and class $j$ at time $t$. We then sample N classes as a task with a probability proportional to their N-cliques potentials, which is expressed as
% % \begin{equation}
% %     P(\mathcal{T})\propto \prod_{i,j\in\mathcal{T}}C^{(t)}(i,j).
% % \end{equation}
% % We sample $K$ such tasks to build $\mathcal{T}^{(t)}$ at each time step $t$.

% \textbf{K-means task clustering}$\quad$The sampled tasks, although are diverse in feature representation, however, are not
% these sampled tasks can still be redundant in terms of latent concepts~(skills) required for performing successful classification. That said, we propose to further cluster these tasks according their latent skills, and sample each candidate task for the final tree search uniformly form each task cluster, thereby ensuring the explored candidates are the most representative at both the feature representation and task functional levels. To achieve this, we first evaluate the negative log-likelihood~(NLL) of each sampled task under $M$ K-NN classifiers constructed from the CL models $\mathcal{F}^{(t)}_m$, resulting in a $M$-dim latent feature vector for each task. The task clusters are then created by running a K-means clustering algorithm. Finally, we adopt ancestral sampling for choosing each candidate task for simulation in the tree search, i.e., sample a cluster and then a task.\par

% \textbf{Time-evolving data pool}~$\quad$~\chen{need to metnion some ideas on how should we udpate the dataset in the pool based on the current results of task-selection? For example, picking visually/conceptually similar datasets to those often selected by our dynamic task selection pipeline ?}
% \textbf{Heuristic task candidates filtering}$\quad$The performance of continual learning algorithms is known to be influenced by the order of tasks due to the intricate interactions between tasks in a learning sequence, such as forward and backward transfer. Previous studies have reached a consensus that a task sequence with intermediate \textit{similarity} between consecutive tasks results in the most significant forgetting. Therefore, we propose to bias our search space towards tasks in $\mathcal{T}^{(t)}$ that exhibit higher similarity to those encountered before $t$, thereby reducing the candiate space for searching for each move. This is accomplished by choosing the Top-$\tilde{K}$, with $\tilde{K}<K$, tasks with classes that have the highest class-pair potential with their closest classes in the past tasks, defined as
% \begin{equation}
%     P(\mathcal{T}\in\mathcal{T}^{(t)})\propto \prod_{i\in\mathcal{T}^{(t)}}\min_{j\in\mathcal{T}^{<(t)}} C^{(t)}(i,j).
% \end{equation}
% After this step, we have reduced the number of plausible actions (the number of candidate tasks) to $\tilde{K}$.\par

% \textbf{Value backpropagation}$\quad$We break down the reward $\gV$ at the terminal state into two components. Firstly, the reward should directly indicate the continual learner's performance, so selecting more challenging task sequences for the learners inherently leads to actions that result in decreased continual learning performance - a standard forgetting metric will be employed for this part. Secondly, \chen{gMAD is used for selecting tasks that lead to maximum disagreement between predictions by different learners. However, how does prediction diversity relate to the continual learning evaluation criteria/goal?}





==> sections/table1_no_robustness.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]\small
  \centering
  \caption{Final average accuracy ($\%$) of CL methods for class-incremental continual learning on different benchmarks. $^\ddagger$ are directly taken from published results. The last two rows show the correlation of evaluation results of different benchmarks with Heldout measured by Spearman’s Rank Correlation  ($\rho$) and Kendall’s ($\tau$). Meanings of `ns' and '$*$' are consistent with Fig~\ref{fig: motivation}. }
  % \resizebox{0.9\textwidth}{!}{
\setlength{\tabcolsep}{1.9mm}{
    \begin{tabular}{lcccc}
    \toprule
    \multirow{2}{*}{\textbf{Method}} &\multicolumn{4}{c}{\textbf{Benchmark}}\\
    \cmidrule(lr){2-5}
          & \textbf{CIFAR-100}$^\ddagger$  & \textbf{ImageNet-R}$^\ddagger$  & \textbf{CLDyB-seq~(Ours)} & \textbf{Heldout} \\
    \cmidrule(lr){1-1}\cmidrule(lr){2-5}
    RanPAC~\citep{mcdonnell2024ranpac} & 92.2  & \textbf{78.1}  & 56.9  & 81.0 \\
    HidePrompt~\citep{wang2023hierarchical} & \textbf{92.6}  & 75.1  & \textbf{62.5}  & \textbf{84.9} \\
    DualPrompt~\citep{Wang2022DualPromptCP} & 86.5  & 68.1  & 41.9  & 70.8 \\
    PGP~\citep{qiao2024promptgrad}   & 86.9  & 69.3  & 44.0  & 68.7 \\
    LAE~\citep{Gao2023AUC}   & 85.6  & 72.7  & 48.1  & 71.1 \\
    SLCA~\citep{Zhang2023SLCASL}  & 91.5  & 77.0  & 56.2  & 80.3 \\
    ER (1000)~\citep{Rolnick2018ExperienceRF} & 67.9  & 55.1  & 54.8  & 79.9 \\
    \cmidrule(lr){1-1}\cmidrule(lr){2-5}
    \textbf{Spearman's}~$\boldsymbol{\rho}$ (per column $\&$ Heldout) & 0.643 (ns) & 0.643 (ns) & \textbf{0.964} $*$ &  N/A  \\
    % \cmidrule(lr){1-1}\cmidrule(lr){2-5}
    \textbf{Kendall's}~$\boldsymbol{\tau}$ (per column $\&$ Heldout) & 0.429 (ns) & 0.429 (ns) & \textbf{0.905} $*$ &  N/A  \\
\bottomrule
    \end{tabular}%
}
  \label{tab: ranking}%
\end{table}%

